IoT Device Identification Based on Network Traffic Characteristics

IoT device identification plays an important role in monitoring and improving the performance and security of IoT devices. Compared to traditional non-IoT devices, IoT devices provide us with both unique challenges and opportunities in detecting the types of IoT devices. Based on critical insights obtained in our previous work on understanding the network traffic characteristics of IoT devices, in this paper we develop an effective machine-learning based IoT device identification scheme, named iotID. In developing iotID, we extract 70 features of TCP flows from three complementary aspects: remote network servers and port numbers, packet-level traffic characteristics such as packet inter-arrival times, and flow-level traffic characteristics such as flow duration. Different from existing work, we take into account the imbalance nature of network traffic generated by various devices in both the learning and evaluation phases of iotID. Our performance studies based on network traffic collected on a typical smart home environment consisting of both IoT and non-IoT devices show that iotID can achieve a balanced accuracy score of above 99%.

==> 04_data_collection.tex <==
\section{Data processing and feature extraction}
In this section we will describe the techniques we adopted to collect the data from the devices as well as the features we extracted from the raw traffic for our studies.



% \begin{table}[]
%     \caption{Number of devices and records}
%     \label{tab:num_devices_records}
%     \centering
%     \begin{tabular}{|>{\raggedright\arraybackslash}m{1.0cm}|>{\raggedright\arraybackslash}m{1.0cm}|>{\raggedright\arraybackslash}m{1.0cm}|>{\raggedright\arraybackslash}m{1.0cm}|}
%         \hline
%         Device & \# of devices & \# of records & \% records \\
%          \hline
%          non-IoT & $7$ & $253,325$ & $90.58$ \\
%          \hline
%          IoT & $12$ & $26,354$ & $9.42$ \\
%          \hline
%          Total & $19$ & $279,679$ & $100$ \\
%          \hline
         
%     \end{tabular}
% \end{table}

\subsection{Feature Extraction}


% 
% We have used both packet level and flow level characteristics for our studies to get optimal performance from the machine learning models. Flow level features include flow duration, remote IP and port, number of packets and bytes, packets and bytes per second. We have used the BGP prefix of the remote IP because the IP address might be random for a particular server. We want to mention that we consider bidirectional flow specifications for all packet or flow level features.

% 




==> 07_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper we analyzed the network traffic characteristics of IoT devices collected on a typical smart home environment consisting of a set of common IoT (and non-IoT) devices. We analyzed the network traffic characteristics of IoT devices from three complementary aspects: remote network servers, flow-level traffic characteristics, and packet-level traffic characteristics.  Our study provided critical insights into the operational and behavioral characteristics of IoT devices, which could have important implications on developing effective security and performance algorithms for IoT devices.
